Incremental Dead State Detection in Logarithmic Time

Identifying live and dead states in an abstract transition system is a recurring problem in formal verification; for example, it arises in our recent work on efficiently deciding regex constraints in SMT. However, state-of-the-art graph algorithms for maintaining reachability information incrementally (that is, as states are visited and before the entire state space is explored) assume that new edges can be added from any state at any time, whereas in many applications, outgoing edges are added from each state as it is explored. To formalize the latter situation, we propose guided incremental digraphs (GIDs), incremental graphs which support labeling closed states (states which will not receive further outgoing edges). Our main result is that dead state detection in GIDs is solvable in $O(\log m)$ amortized time per edge for $m$ edges, improving upon $O(\sqrt{m})$ per edge due to Bender, Fineman, Gilbert, and Tarjan (BFGT) for general incremental directed graphs. We introduce two algorithms for GIDs: one establishing the logarithmic time bound, and a second algorithm to explore a lazy heuristics-based approach. To enable an apples-to-apples experimental comparison, we implemented both algorithms, two simpler baselines, and the state-of-the-art BFGT baseline using a common directed graph interface in Rust. Our evaluation shows $110$-$530$x speedups over BFGT for the largest input graphs over a range of graph classes, random graphs, and graphs arising from regex benchmarks.

==> app.tex <==

\section{Appendix}

\subsection{Extension to the Framework: Non-Reachable Updates}
\label{subsec:non-reachable}

When GIDs are viewed as an abstract data type, other application-specific heuristics can be incorporated.
To illustrate this point, we consider another piece of application-specific information: assertions which state that one state is not (and will never be) reachable from another.
We discuss how to incorporate such updates to further improve the optimized algorithm in practice to exploit such updates.

First, we augment the definition of guided incremental digraph
to allow updates of the form $\code{N}(u, v)$, which labels that $v$ is not reachable from $u$.
We then say that the graph is \emph{valid} if, in addition to the previous conditions, for every update $\code{N}(u, v)$, $v$ is not reachable from $u$ via a sequence of edges in the final digraph.
\Cref{ex:gid-3} extends the example presented in \Cref{ex:gid-1,ex:gid-2} with a not-reachable update.
Notice that $\code{N}(3, 5)$ does not affect the set of live and dead states,
but may be exploited for more efficient search.

To incorporate $\code{N}(u, v)$ updates in our algorithm,
when moving a reserve edge into the graph, $\code{N}(u, v)$ can be used to shortcut the whole procedure: if we add an edge $(v, u)$ in particular, then we know that this does not create a cycle, and we don't need to repeatedly call $\code{succ}{z}$ at all.
We store $\code{N}(u, v)$ updates in a set instead of a list for $O(1)$ querying; if we need to merge them, we just discard the set if it gets too large.
Therefore, in addition what was maintained previously, the extended algorithm tracks, for each unknown canonical state $x$, a set of \emph{non-reachable} edges $(x, y)$, where each corresponds to some update $\code{N}(u, v)$ with $x = \code{find}(u)$ and $y = \code{find}(v)$ (but not necessarily vice versa);
and a constant $\kappa$ which bounds the amount of work when merging non-reachable sets (additional elements will be discarded).
We modify the code for $\code{is-root}(y, x)$ with a single check
in the beginning of the procedure: if $x$ is in the not-reachable set from $y$, return false. Otherwise, we continue as normal.
Because this algorithm uses the $\code{N}(u, v)$ information directly and conservatively, assuming the input GID is valid, it remains correct.

\begin{figure}[t]
\centering
\begin{tikzpicture}
\node[state, open] (q1) {$1$};
\node[state, below left of=q1, accepting] (q2) {$2$};
\node[state, below right of=q1, open] (q3) {$3$};
\node[state, above right of=q3] (q4) {$4$};
\node[state, below right of=q4] (q5) {$5$};
\draw (q1) edge (q2);
\draw (q1) edge (q3);
\draw (q4) edge (q3);
\draw (q4) edge (q5);
\draw (q3) edge[dashed, color=red] (q5);
\end{tikzpicture}
\caption{
Extension to our framework:
guided incremental digraph from \Cref{ex:gid-1,ex:gid-2},
with an added update $\code{N}(3, 5)$
which states that $5$ is not reachable from $3$.
In this graph, it would be invalid to then add $\code{E}(3, 4)$ to the graph.
This does not change the set of live or dead states, but may
be exploited for more efficient search:
when checking if state $3$ is live or dead,
we may ignore states $4$ and $5$.
}
\label{ex:gid-3}
\end{figure}

\subsection{Reachability Problems on EREs}

For extended regexes $X$ and $Y$,
we say that $Y$ is \emph{reachable} from $X$ if $Y \in \DERIVT(X)$.
We say that $X$ and $Y$ are \emph{strongly
  connected}, denoted $X\SC Y$, when both $Y\in \DERIVT(X)$ and $X\in
\DERIVT(Y)$, i.e., when both $Y$ is reachable from $X$ and $X$ is
reachable from $Y$ through derivation as defined above.

We also consider the following subclasses of extended regexes:
\begin{itemize}
    \item \emph{Regexes (REs)} are EREs that do not contain complement or intersection, that is, classical regexes.
    \item \emph{Semi-extended regexes (SEREs)} are EREs that do not contain complement.
    \item \emph{Intersections of regexes (IREs)} are SEREs that are equal to an intersection of REs.
    \item \emph{Boolean combinations of regexes (BCREs)} are EREs that are equal to a Boolean combination (combination of intersection and complement) of REs.
\end{itemize}
Semantically, all of these capture the set of regular languages.
The syntactic relationships between these different subclasses is summarized as follows,
where all inclusions are strict:
\[
\begin{array}{ccccc}
\text{RE} & \subset & \text{IRE} & \subset & \text{BCRE} \\
    && \cap && \cap \\
    && \text{SERE} & \subset & \text{ERE}
\end{array}
\]

We consider the following three decision problems.
They are closely related and in order of generality: the first is a special case of both the second and thirds, and the second reduces to two queries of the third.
For each problem, we also consider problems on all the subclasses of EREs that we defined: REs, SEREs, IREs, and BCREs.
We summarize the complexity results in the table in
\Cref{fig:regex-complexity-results}.

\begin{description}
\item[Edge in Cycle:] Given $X$ and $Y$ such that $X \in \DERIV(Y)$, is $Y \in \DERIVT(X)$?
\item[Strong Connectedness:] Given $X$ and $Y$, is $X \SC Y$?
\item[Reachability:] Given $X$ and $Y$, is $Y \in \DERIVT(X)$?
\end{description}

\begin{figure}[t]
\centering
\begin{tabular}{ccccccc}
\toprule
Subclass & \phantom{a} & Edge in Cycle & \phantom{a} & Strong Connectedness & \phantom{a} & Reachability \\
\cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-7}
RE
    && Linear && Linear && Linear \\
IRE
    && PSPACE-C && PSPACE-C && PSPACE-C \\
BCRE
    && PSPACE-C && PSPACE-C && PSPACE-C \\
SERE
    && PSPACE-C && PSPACE-C && PSPACE-C \\
ERE
    && non-elementary && non-elementary && non-elementary \\
\bottomrule
\end{tabular}
\caption{Complexity results for reachability of various subclasses of extended regexes.}
\label{fig:regex-complexity-results}
\end{figure}

The first result below is likely known, but we include a proof.

\begin{theorem}
For RE, the edge-in-cycle, strong-connectedness, and reachability problems can be solved in linear time.
\end{theorem}
\begin{proof}
It suffices to show that reachability can be solved in linear time,
since as stated above, it is the most general of the three.
We give a decision procedure for deciding $Y \in \DERIVT(X)$ by recursing on the structure of $X$.
Prior to the procedure, we ensure (i) that all regexes are normalized, (ii) that equal regexes are represented by the same pointer, and (iii) that concatenations are represented as cons lists and precompute the length of each list, so that for any subexpression $X_0$ of $X$, whether $Y = Y_1 \cdot X_0$ can be checked in constant time.
This precomputation takes $O(|X| + |Y|)$ time.
The recursion then works as follows, on input $(X, Y)$. (1) If $X = \varphi$, $\eps$, or $\emp$, we can check directly if $Y$ is one of the finitely many derivatives. (2) If $X = X_1 \ror X_2$, we observe that $Y \in \DERIVT(X)$ if and only if $Y \in \DERIVT(X_1)$ or $Y \in \DERIVT(X_2)$.
So we recurse on $(X_1, Y)$ and $(X_2, Y)$.
(3) If $X = X_1^*$, we observe that $Y \in \DERIVT(X)$ if and only if $Y = X_1' (X_1^*)$ for $X_1' \in \DERIVT(X_1)$.
So we first check if $Y$ has the form $Y_1 X_1^*$, then recurse on $(X_1, Y_1)$.
(4) Finally, if $X = X_1 \cdot X_2$, we observe that $Y \in \DERIVT(X)$ if and only if either $Y = X_1' \cdot X_2$ for $X_1' \in \DERIVT(X_1)$, or $Y = X_2'$ for $X_2' \in \DERIVT(X_2)$. (Note that this relies on the fact that $X_1$ is an RE, not an ERE, so we know it is nonempty and in particular there is some nullable $R \in \DERIVT(X_1)$.)
So we first check if $Y$ has the form $Y_1 \cdot X_2$, if so recursing on both $(X_1, Y_1)$ and $(X_2, Y)$, otherwise recursing on just $(X_2, Y)$.
Since the procedure never recurses twice on $X$ or twice on the same subexpression of $X$,
it takes $O(|X|)$ time.
\qed
\end{proof}

\begin{theorem}
For the classes IRE, BCRE, and SERE, the edge-in-cycle, strong-connectedness, and reachability problems are PSPACE-complete.
\end{theorem}
\begin{proof}
It suffices to show: (1) the edge-in-cycle problem for IRE is PSPACE-hard; (2)
the reachability problem for BCRE is in PSPACE; and (3) the reachability problem for SERE is in PSPACE.
\textbf{(1)} We reduce from intersection-nonemptiness of REs, which is known to be PSPACE-hard.
Given a list of REs $R_1, R_2, \ldots, R_k$, then let $b$ be a fresh character
that does not appear in $R_1, \ldots, R_k$, and construct the IRE
$X = (b R_1)^* \rand (b R_2)^* \rand \cdots \rand (b R_k)^*.$
$X$ has only one derivative $X'$, which is an intersection where the $i$th term is
$R_i (b R_i)^*$.
Then the edge-in-cycle property for $(X', X)$ holds if and only if the intersection of
$R_i$ is nonempty, because $\deriv[b]{}$ is empty for all subexpressions of $R_i$, so the only way to get back to $X$ is by stepping all $R_i$ to $\eps$ simultaneously.
\textbf{(2)}
TODO
\textbf{(3)} For an SERE $X$, for any $X' \in \DERIVT(X)$ we show that the size of $X'$ is bounded linearly in the size of the $X$. This can be seen by induction on the structure of $X$; for example, elements of $\DERIVT(X_1 \rand X_2)$ are a pair of an element of $\DERIVT(X_1)$ and an element of $\DERIVT(X_2)$.
It follows that we can provide the following NPSPACE algorithm for reachability of $(X, Y)$: at each step, pick a derivative nondeterministically of $X$ and recurse.
\qed
\end{proof}

\begin{theorem}
For ERE, the edge-in-cycle, strong-connectedness, and reachability problems are non-elementary.
\end{theorem}
\begin{proof}
It suffices to show that the edge-in-cycle problem is non-elementary. We reduce from the nonemptiness problem for EREs, which is known to be non-elementary~\cite{stockmeyer1973word}.
Given an ERE $R$, we let $b$ be a fresh character not appearing in $R$,
and we let $X = (bR)^*$.
Then $X$ has one derivative, $X' = R(bR)^*$.
The edge-in-cycle property for $(X', X)$ holds and only if $R$ is nonempty,
because some element of $\DERIVT(R)$ will be nullable.
\qed
\end{proof}



